Concatenated Power Mean Word Embeddings as Universal Cross-Lingual Sentence Representations

Average word embeddings are a common baseline for more sophisticated sentence embedding techniques. However, they typically fall short of the performances of more complex models such as InferSent. Here, we generalize the concept of average word embeddings to power mean word embeddings. We show that the concatenation of different types of power mean word embeddings considerably closes the gap to state-of-the-art methods monolingually and substantially outperforms these more complex techniques cross-lingually. In addition, our proposed method outperforms different recently proposed baselines such as SIF and Sent2Vec by a solid margin, thus constituting a much harder-to-beat monolingual baseline. Our data and code are publicly available.

==> evaluation.tex <==
\section{Experimental Setup}\label{sec:evaluation}

\begin{table*}
\centering
\footnotesize
\begin{tabular}{llcccl}
\toprule
\textbf{Task} & \textbf{Type} & \textbf{Size} & \textbf{X-Ling} & \textbf{C} & \textbf{Example} \\ 
\midrule
AM & Argumentation & 7k  & H+MT & 4 & Viele der technologischen Fortschritte helfen der Umwelt sehr.  \textit{(claim)} 
 \\
AMicro & Argumentation & 450 & H+MT & 2 & Too many promises have not been kept. \textit{(none)} \\
CLS & Product-reviews & 6k & H & 2 & En tout cas on ne s'ennuie pas à la lecture de cet ouvrage! \textit{(pos)} \\
\midrule 
MR & Sentiment & 11k & MT & 2 & Dunkel und verstörend, aber auch überraschend witzig. \textit{(pos)} \\
CR & Product-reviews & 4k & MT & 2 & This camera has a major design flaw. \textit{(neg)} \\
SUBJ & Subjectivity & 10k & MT & 2 & On leur raconte l'histoire de la chambre des secrets. \textit{(obj)} \\
MPQA & Opinion-polarity & 11k & MT & 2 & sind eifrig \textit{(pos)} $|$ nicht zu unterstützen \textit{(neg)} \\
TREC & Question-types & 6k & MT & 6 & What's the Olympic Motto? \textit{(desc)} \\
SST & Sentiment & 70k & MT & 2 & Holm... incarne le personnage avec un charisme regal [...] \textit{(pos)} \\
\bottomrule
\end{tabular}
\caption{The evaluation tasks with examples from different languages. While the first three tasks contain human-generated cross-lingual data (H), we translated all sentences for the last 6 tasks using Google Translate (MT). The column C denotes the number of classes.}
\label{table:evaluation:tasks}
\end{table*}

\subsection{Tasks}
\paragraph{Monolingual}
The goal of `universal sentence embeddings' is to yield stable and high-performing results across a wide range of so-called transfer tasks. To measure whether our sentence embeddings satisfy this criterion, we replicate the same setup as in \newcite{Conneau2017} and evaluate on the six transfer tasks listed in their table 1.

Noting that their tasks are somewhat biased towards sentiment analysis, we introduce three additional tasks to evaluate universal sentence embeddings: (1) \textit{AM}, an argumentation mining task based on \newcite{Stab:2017} where sentences are classified into the categories major claim, claim, premise, and non-argumentative; (2) \textit{AMicro}, a further argumentation mining classification task with very few data points based on \newcite{Peldszus2016} in which the goal is to classify sentences as to whether they contain a claim or not \cite{Daxenberger:2017}; (3) \textit{CLS}, a task based on the XY dataset \cite{} to identify individual sentences as being part of a positive or negative book review.

With the addition of our own tasks, we extend the evaluation of sentence embeddings with a new domain and a scenario with very few data points. We summarize properties of our tasks in Table \ref{table:evaluation:tasks}.

\paragraph{Cross-lingual datasets}

Sentences in \textit{AMicro} (en-de)
are already parallel, having been (semi-)professionally translated by humans from the original English. 
For \textit{AM}, we have access to human student translations from the original English into German. 
\textit{CLS} (en-de,en-fr) is also available bilingually. 
In addition, 
we created machine translated versions for all datasets (even those that already have human translations) using Google Translate for the directions en-de and en-fr.

In total, we collected XXX human-generated sentences and YYY machine-translated sentences for our transfer languages. 

\subsection{Word embeddings}
\paragraph{Monolingual}

We use four diverse, potentially complementary types of word embeddings %to create our sentence 
as basis for our sentence
representation techniques:
(1) GloVe embeddings \cite{Pennington2014} trained on Common Crawl;
(2) Word2Vec \cite{Mikolov2013} trained on the Google News corpus; (3) Attract-Repel \cite{Mrksic2017}, which are designed to differentiate between antonyms; 
(4) MorphSpecialized \cite{Vulic2017}, which are designed to differentiate between inflectional forms and derivational antonyms. We use pre-trained variants of the embedding types (1),(2),(4) and for (3) we use the retrofitting code provided by the authors\footnote{https://github.com/nmrksic/attract-repel} to tune the embeddings of \newcite{Komninos:2016}.


\paragraph{Cross-lingual}
Since our above embeddings are not all available cross-lingually, we use alternatives where necessary:

(1) 
We train en-de and en-fr BIVCD embeddings on aligned sentences from the Europarl \cite{Koehn:2005} and the UN corpus \cite{Ziemski:2016}, respectively, using word2vec \cite{Mikolov2013}; (2) Attract-Repel (AR) \cite{Mrksic2017} provide pre-trained cross-lingual word embeddings for en-de and en-fr; 
(3) Monolingual Fasttext word embeddings \cite{Bojanowski2017} of multiple languages 
trained on Wikipedia, which we map into shared vector space with our method described in §\ref{sec:xling-mapping}. We also re-map the BIVCD and AR embeddings using our technique. Even though BIVCD performances were not affected by this projection, AR embeddings were greatly improved by it. \todo{SE: describe monolingual fasttex in the related work section}

All our word embeddings, whether mono- or cross-lingual, have dimensionality $d'=300$. 

\subsection{Evaluated Approaches}
\paragraph{Monolingual}

For each type of word embedding, we evaluate the
standard average word embedding ($p=1$) as sentence embedding as well as different concatenations of embeddings. 
We also evaluate concatenations of embeddings $\mathbf{s}^{(i)}(1,\infty,-\infty)$, where $i$ ranges over our four type of embeddings mentioned above.\footnote{In the monolingual setup, we limit our experiments to %three $p$-means to keep 
the three named $p$-means so that 
dimensionality 
does not exceed that of InferSent. 
See Section \ref{sec:discussion:p-values} for a further comparison of different $p$-values.} Thus, the maximum dimensionality of our sentence embeddings is $d=4\cdot 3\cdot 300=3600$. 
%
We compare our representations
against SIF, which may be perceived of as a direct competitor, as well as InferSent, which constitutes the state-of-the-art and which was shown to outperform many strong baselines such as Skip-thought in \newcite{Conneau2017}.


\paragraph{Cross-lingual}

Similar to the monolingual case, we evaluate standard averages ($p=1$) for all word embedding types, 
as well as different concatenations and $p$-means.
Since we have only three rather than four base embeddings here, 
we directly additionally report results for $p=3$.\footnote{$p=3$ has the advantage over $p=2$ that it preserves sign information.}

Additionally, 
we also report performances of bilingual SIF embeddings, i.e., SIF applied to bilingual word embeddings, and 
three novel cross-lingual variants of InferSent:

(1) \textit{InferSent MT}: We translated all 569K sentences in the SNLI corpus \cite{Bowman:2015} 
to German and French using Google Translate. 
To train, e.g., en-de InferSent, we consider all 4 possible language combinations over each sentence pair in the SNLI corpus, i.e., if $(u,v)$ is in the original corpus, then our bilingual SNLI corpus has pairs $(u_{s},v_{t})$ where $s,t$ range over English and German. 
Thus, we infer four new cross-lingual training samples from one original data point, and therefore our new SNLI corpus is four times as large as the original.

(2) \textit{InferSent TD}: We formulate a different task where the InferSent model has to differentiate between translations and unrelated sentences (translation detection), i.e., the model has two output classes but is otherwise the same architecture. To obtain translations, we use sentence translation pairs from Europarl (de) and the UN corpus (fr); unrelated sentences were randomly sampled from the respective corpora. We limited the number of training samples to the size of the SNLI corpus to keep the training time reasonable. 

(3) \textit{InferSent MT+TD}: This is a combination of the two previous approaches where we merge translation detection data with cross-lingual SNLI. Even though translations are similar to entailment relations, and unrelated sentences are similar to neutral relations, we do not map the two label sets for two reasons. First, translations carry the exact same meaning in a bilingual context (are symmetric) while entailments are strictly unidirectional (are non-symmetric). Second, neutral sentences from SNLI are usually topically related, but unrelated sentences from the translation detection cover different topics. 

We trained all InferSent adaptations using the best-performing word embeddings as input (the ones that achieved the highest performance in our evaluations) to provide a fair (even slightly biased) comparison.

\subsection{Evaluation Procedure}
It is common practice to use the 
simplest classification approach for the evaluation of sentence embeddings in order to minimize potential influences from the classifier and only evaluate the embeddings themselves. We adhere to this standard by training a logistic regression classifier on top of our sentence embeddings for our newly added tasks. Furthermore, we use random subsample validation \cite{} in order to mitigate the effects of different random initializations of the weight vector in logistic regression with 50 runs for each model. We use SGD with the Adam optimizer \cite{Kingma2015} and perform grid search for the learning rate due its noticeable impact on the results. 

To allow for a direct comparison against previously published results, we use the SentEval framework \cite{Conneau2017} for the tasks MR, CR, SUBJ, MPQA, TREC, and SST. For most tasks, this approach likewise uses logistic regression with 10-fold cross validation and no further optimization of the learning rate.

We report macro F1 performance for our own tasks to account for imbalanced classes, and accuracy for all tasks evaluated using SentEval.

In the bilingual setup we apply the same evaluation procedure as in the monolingual one and train the classifiers on English sentence embeddings. However, we then measure the transfer performance on German and French sentences.


==> results.tex <==
\section{Results}
\input{tables/monolingual-results}
\paragraph{Monolingual}
The results of Table \ref{table:results:monolingual} show that we can substantially improve sentence embeddings when concatenating multiple word embedding types. This is the case for both the arithmetic mean and other $p$-mean values, indicating that different types of word embeddings indeed contain complementary information. With all four embedding types concatenated, we achieve a 2pp improvement over the best individual embeddings (Glove). 
All sentence embeddings also perform substantially better when incorporating further power mean values. Glove improves by 0.6pp on average, GoogleNews by 1.9pp, MS by 2.1pp and AR by 3.7pp when concatenating $p=\pm\infty$ to the standard value of $p=1$ (dimensionality increase from $300$ to $900$). 

The combination of concatenation and power means gives an average improvement of 3pp over the individually best embedding type. With this, we reduce the gap to InferSent from 4.6pp to 1.6pp, which closes the gap by 60\%, while still having a lower dimensionality (3600 vs. 4096).

We also consistently outperform SIF and Sent2Vec.


\paragraph{Cross-lingual}
\input{tables/crosslingual-results-avg}

For ease of consideration, 
we report here average results 
over en$\rightarrow$de and en$\rightarrow$fr in Table \ref{table:results:x-ling}. 
Scores for the individual languages can be found in Appendix \ref{appendix:fine-grained-results}.

As in the monolingual case, we observe  substantial improvements when concatenating different types of word embeddings of $\sim$2pp on average.
When adding FT embeddings to the already strong concatenation of BV and AR, however, the cross-lingual performance only slightly improves on average while the monolingual performance increase is more pronounced. 
This may suggest that the monolingual gain 
cannot be fully transfered across languages here.

Conversely, using different $p$-means is more substantially effective, considerably improving 
performance values compared to the arithmetic mean word embeddings. 
In particular, we notice that employing $p$-means with AR word embeddings yields a performance gain similar to using X-InferSent-MT (due to a higher cross-language drop). 
On average, concatenation plus different power means beats the best individual word embeddings by 4.4\% points (dimensionality of $3600$) cross-lingually. 

Cross-lingually we not only beat all our InferSent adaptations by more than 2pp on average, 
our concatenated $p$-mean embeddings also outperform the more complex InferSent adaptations 
in almost all individual transfer tasks (8 out of 9).



